A 4 Gyr M-dwarf Gyrochrone from CFHT/MegaPrime Monitoring of the Open Cluster M67

We present stellar rotation periods for late K- and early M-dwarf members of the 4 Gyr old open cluster M67 as calibrators for gyrochronology and tests of stellar spin-down models. Using Gaia EDR3 astrometry for cluster membership and Pan-STARRS (PS1) photometry for binary identification, we build this set of rotation periods from a campaign of monitoring M67 with the Canada-France-Hawaii Telescope's MegaPrime wide field imager. We identify 1807 members of M67, of which 294 are candidate single members with significant rotation period detections. Moreover, we fit a polynomial to the period versus color-derived effective temperature sequence observed in our data. We find that the rotation of very cool dwarfs can be explained by a simple solid-body spin-down between 2.7 and 4 Gyr. We compare this rotational sequence to the predictions of gyrochronological models and find that the best match is Skumanich-like spin-down, P_rot \propto t^0.62, applied to the sequence of Ruprecht 147. This suggests that, for spectral types K7-M0 with near-solar metallicity, once a star resumes spinning down, a simple Skumanich-like is sufficient to describe their rotation evolution, at least through the age of M67. Additionally, for stars in the range M1-M3, our data show that spin-down must have resumed prior to the age of M67, in conflict with predictions of the latest spin-down models.

==> M67 Rotation Periods/figure_set.tex <==
\figsetstart
\figsetnum{16}
\figsettitle{Light Curves and Periodograms}

\figsetgrpstart
\figsetgrpnum{16.1}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598696107233137920}
\figsetplot{598696107233137920.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.2}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598696833082561280}
\figsetplot{598696833082561280.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.3}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598697103669936512}
\figsetplot{598697103669936512.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.4}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598883642685066368}
\figsetplot{598883642685066368.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.5}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598883917565244288}
\figsetplot{598883917565244288.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.6}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598883990577158400}
\figsetplot{598883990577158400.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.7}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598885085794212096}
\figsetplot{598885085794212096.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.8}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598885090090313216}
\figsetplot{598885090090313216.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.9}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598885502406044544}
\figsetplot{598885502406044544.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.10}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598886082226539136}
\figsetplot{598886082226539136.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.11}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598886288384971008}
\figsetplot{598886288384971008.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.12}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598886911154739968}
\figsetplot{598886911154739968.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.13}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598887216100088192}
\figsetplot{598887216100088192.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.14}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598887254752714240}
\figsetplot{598887254752714240.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.15}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598887632709845248}
\figsetplot{598887632709845248.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.16}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598887770148211584}
\figsetplot{598887770148211584.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.17}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598888109451094912}
\figsetplot{598888109451094912.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.18}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598888315613964288}
\figsetplot{598888315613964288.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.19}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598888521767965568}
\figsetplot{598888521767965568.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.20}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598888727926385408}
\figsetplot{598888727926385408.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.21}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598889213257785984}
\figsetplot{598889213257785984.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.22}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598894569081905920}
\figsetplot{598894569081905920.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.23}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598899997920577664}
\figsetplot{598899997920577664.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.24}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598900105294874496}
\figsetplot{598900105294874496.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.25}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598900753834826880}
\figsetplot{598900753834826880.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.26}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598901269230913024}
\figsetplot{598901269230913024.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.27}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598902540541250944}
\figsetplot{598902540541250944.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.28}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598903055937325312}
\figsetplot{598903055937325312.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.29}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598903090297061760}
\figsetplot{598903090297061760.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.30}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598903674412626432}
\figsetplot{598903674412626432.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.31}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598903987945320832}
\figsetplot{598903987945320832.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.32}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598905667277445376}
\figsetplot{598905667277445376.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.33}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598906290047773440}
\figsetplot{598906290047773440.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.34}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598906835508558336}
\figsetplot{598906835508558336.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.35}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598906942882791424}
\figsetplot{598906942882791424.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.36}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598907179105947520}
\figsetplot{598907179105947520.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.37}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598907969381972864}
\figsetplot{598907969381972864.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.38}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598908042394421248}
\figsetplot{598908042394421248.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.39}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598908248552758400}
\figsetplot{598908248552758400.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.40}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598908278617636608}
\figsetplot{598908278617636608.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.41}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598947517438273792}
\figsetplot{598947517438273792.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.42}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598953770910670336}
\figsetplot{598953770910670336.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.43}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598955385818884096}
\figsetplot{598955385818884096.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.44}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598955660696788736}
\figsetplot{598955660696788736.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.45}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598955729416446208}
\figsetplot{598955729416446208.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.46}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598956382253218816}
\figsetplot{598956382253218816.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.47}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598956450970778624}
\figsetplot{598956450970778624.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.48}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598956485330513536}
\figsetplot{598956485330513536.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.49}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598956523984534272}
\figsetplot{598956523984534272.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.50}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598956833222201216}
\figsetplot{598956833222201216.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.51}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598957279899423232}
\figsetplot{598957279899423232.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.52}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598957756640350080}
\figsetplot{598957756640350080.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.53}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598957756642455680}
\figsetplot{598957756642455680.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.54}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598958512554598400}
\figsetplot{598958512554598400.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.55}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598959371548060672}
\figsetplot{598959371548060672.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.56}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598959513281774208}
\figsetplot{598959513281774208.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.57}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598970366666045952}
\figsetplot{598970366666045952.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.58}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598970645837645440}
\figsetplot{598970645837645440.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.59}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598970886355816320}
\figsetplot{598970886355816320.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.60}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598977513489950592}
\figsetplot{598977513489950592.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.61}
\figsetgrptitle{Light curve and periodogram of Gaia ID 598977547849690496}
\figsetplot{598977547849690496.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.62}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604686422674966912}
\figsetplot{604686422674966912.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.63}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604687006790507904}
\figsetplot{604687006790507904.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.64}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604687178590760192}
\figsetplot{604687178590760192.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.65}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604698860900256256}
\figsetplot{604698860900256256.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.66}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604699479375624320}
\figsetplot{604699479375624320.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.67}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604701747118303104}
\figsetplot{604701747118303104.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.68}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604703465105196416}
\figsetplot{604703465105196416.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.69}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604703636903893504}
\figsetplot{604703636903893504.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.70}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604704010566644480}
\figsetplot{604704010566644480.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.71}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604706862424426496}
\figsetplot{604706862424426496.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.72}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604709134461425024}
\figsetplot{604709134461425024.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.73}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604711913305981952}
\figsetplot{604711913305981952.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.74}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604712188183890304}
\figsetplot{604712188183890304.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.75}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604712531781276928}
\figsetplot{604712531781276928.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.76}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604712600500056320}
\figsetplot{604712600500056320.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.77}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604713532508424448}
\figsetplot{604713532508424448.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.78}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604713669947377024}
\figsetplot{604713669947377024.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.79}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604736136920843648}
\figsetplot{604736136920843648.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.80}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604736308719544960}
\figsetplot{604736308719544960.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.81}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604736690972080512}
\figsetplot{604736690972080512.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.82}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604737275087042944}
\figsetplot{604737275087042944.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.83}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604737854908112896}
\figsetplot{604737854908112896.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.84}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604891069277322624}
\figsetplot{604891069277322624.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.85}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604891412874700544}
\figsetplot{604891412874700544.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.86}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604892989128623488}
\figsetplot{604892989128623488.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.87}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604894917568011520}
\figsetplot{604894917568011520.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.88}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604895467323840256}
\figsetplot{604895467323840256.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.89}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604895673481330688}
\figsetplot{604895673481330688.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.90}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604896115863131776}
\figsetplot{604896115863131776.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.91}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604896463756224640}
\figsetplot{604896463756224640.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.92}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604896498115959296}
\figsetplot{604896498115959296.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.93}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604896528179994240}
\figsetplot{604896528179994240.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.94}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604896631259208192}
\figsetplot{604896631259208192.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.95}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604896631259520512}
\figsetplot{604896631259520512.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.96}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604896807353611264}
\figsetplot{604896807353611264.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.97}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604896979152285056}
\figsetplot{604896979152285056.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.98}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604897146655294976}
\figsetplot{604897146655294976.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.99}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604897696411104256}
\figsetplot{604897696411104256.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.100}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604897696411107840}
\figsetplot{604897696411107840.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.101}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604897799490329216}
\figsetplot{604897799490329216.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.102}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604897803785089024}
\figsetplot{604897803785089024.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.103}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604897902569851264}
\figsetplot{604897902569851264.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.104}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604898113023651328}
\figsetplot{604898113023651328.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.105}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604898246166933504}
\figsetplot{604898246166933504.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.106}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604898490980774784}
\figsetplot{604898490980774784.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.107}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604898555404553344}
\figsetplot{604898555404553344.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.108}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604899006376815488}
\figsetplot{604899006376815488.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.109}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604899418693667584}
\figsetplot{604899418693667584.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.110}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604899448757770624}
\figsetplot{604899448757770624.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.111}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604899654921447168}
\figsetplot{604899654921447168.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.112}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604899899730026496}
\figsetplot{604899899730026496.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.113}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604900449485824256}
\figsetplot{604900449485824256.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.114}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604900651348634240}
\figsetplot{604900651348634240.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.115}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604900754427832448}
\figsetplot{604900754427832448.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.116}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604900793084792192}
\figsetplot{604900793084792192.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.117}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604901171040299904}
\figsetplot{604901171040299904.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.118}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604901407262883456}
\figsetplot{604901407262883456.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.119}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604901686436367232}
\figsetplot{604901686436367232.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.120}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604902098753249280}
\figsetplot{604902098753249280.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.121}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604902128817395072}
\figsetplot{604902128817395072.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.122}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604902334975837312}
\figsetplot{604902334975837312.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.123}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604902442350618368}
\figsetplot{604902442350618368.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.124}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604902648509053184}
\figsetplot{604902648509053184.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.125}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604902987810825728}
\figsetplot{604902987810825728.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.126}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604903090890049792}
\figsetplot{604903090890049792.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.127}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604903125251398144}
\figsetplot{604903125251398144.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.128}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604903331408222208}
\figsetplot{604903331408222208.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.129}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604903370063592192}
\figsetplot{604903370063592192.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.130}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604903438783070208}
\figsetplot{604903438783070208.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.131}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604903438783071616}
\figsetplot{604903438783071616.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.132}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604903576222014080}
\figsetplot{604903576222014080.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.133}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604903782380443904}
\figsetplot{604903782380443904.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.134}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604903816740187264}
\figsetplot{604903816740187264.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.135}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604904813174193536}
\figsetplot{604904813174193536.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.136}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604904881892076032}
\figsetplot{604904881892076032.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.137}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604905912684188928}
\figsetplot{604905912684188928.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.138}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604906290641338752}
\figsetplot{604906290641338752.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.139}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604906531159506304}
\figsetplot{604906531159506304.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.140}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604906840397139584}
\figsetplot{604906840397139584.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.141}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604906973546358528}
\figsetplot{604906973546358528.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.142}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604907046555569664}
\figsetplot{604907046555569664.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.143}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604907218354253568}
\figsetplot{604907218354253568.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.144}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604907523302217472}
\figsetplot{604907523302217472.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.145}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604907660735224704}
\figsetplot{604907660735224704.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.146}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604908008628339200}
\figsetplot{604908008628339200.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.147}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604908107412145408}
\figsetplot{604908107412145408.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.148}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604908352225723520}
\figsetplot{604908352225723520.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.149}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604908489664691456}
\figsetplot{604908489664691456.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.150}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604908833261132928}
\figsetplot{604908833261132928.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.151}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604909138204304128}
\figsetplot{604909138204304128.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.152}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604909310002693632}
\figsetplot{604909310002693632.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.153}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604909383016937088}
\figsetplot{604909383016937088.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.154}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604909619240334592}
\figsetplot{604909619240334592.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.155}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604909894118735360}
\figsetplot{604909894118735360.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.156}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604909928477987584}
\figsetplot{604909928477987584.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.157}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604909967133410688}
\figsetplot{604909967133410688.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.158}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604909967133412096}
\figsetplot{604909967133412096.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.159}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604910100276687232}
\figsetplot{604910100276687232.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.160}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604910482529472256}
\figsetplot{604910482529472256.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.161}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604910581313218176}
\figsetplot{604910581313218176.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.162}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604910654328188416}
\figsetplot{604910654328188416.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.163}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604910723047665024}
\figsetplot{604910723047665024.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.164}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604910924910708224}
\figsetplot{604910924910708224.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.165}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604911375881849216}
\figsetplot{604911375881849216.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.166}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604911405946776448}
\figsetplot{604911405946776448.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.167}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604911547681374976}
\figsetplot{604911547681374976.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.168}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604911680824696064}
\figsetplot{604911680824696064.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.169}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604911685120318592}
\figsetplot{604911685120318592.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.170}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604911685120320640}
\figsetplot{604911685120320640.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.171}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604911886983070720}
\figsetplot{604911886983070720.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.172}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604912097436452224}
\figsetplot{604912097436452224.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.173}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604912372315122176}
\figsetplot{604912372315122176.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.174}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604912441036157568}
\figsetplot{604912441036157568.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.175}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604912608537595008}
\figsetplot{604912608537595008.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.176}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604912917781019008}
\figsetplot{604912917781019008.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.177}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604913403107275008}
\figsetplot{604913403107275008.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.178}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604913471826560512}
\figsetplot{604913471826560512.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.179}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604913742408986752}
\figsetplot{604913742408986752.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.180}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604913776768724352}
\figsetplot{604913776768724352.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.181}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604913811128465408}
\figsetplot{604913811128465408.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.182}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604913948567397888}
\figsetplot{604913948567397888.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.183}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604914227740983936}
\figsetplot{604914227740983936.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.184}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604914807561160064}
\figsetplot{604914807561160064.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.185}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604915013719302784}
\figsetplot{604915013719302784.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.186}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604915567770583424}
\figsetplot{604915567770583424.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.187}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604915597835911168}
\figsetplot{604915597835911168.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.188}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604916083166650752}
\figsetplot{604916083166650752.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.189}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604916181950391936}
\figsetplot{604916181950391936.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.190}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604916181950394240}
\figsetplot{604916181950394240.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.191}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604916254965496960}
\figsetplot{604916254965496960.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.192}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604916353749267840}
\figsetplot{604916353749267840.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.193}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604916392404461184}
\figsetplot{604916392404461184.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.194}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604916529843404928}
\figsetplot{604916529843404928.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.195}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604916697346488960}
\figsetplot{604916697346488960.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.196}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604917006584145792}
\figsetplot{604917006584145792.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.197}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604917491916094336}
\figsetplot{604917491916094336.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.198}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604917663714774912}
\figsetplot{604917663714774912.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.199}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604917693779073280}
\figsetplot{604917693779073280.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.200}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604917899937362048}
\figsetplot{604917899937362048.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.201}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604917968656982016}
\figsetplot{604917968656982016.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.202}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604918174815279616}
\figsetplot{604918174815279616.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.203}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604918179110939264}
\figsetplot{604918179110939264.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.204}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604918247830312832}
\figsetplot{604918247830312832.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.205}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604918552772398720}
\figsetplot{604918552772398720.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.206}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604918900665305600}
\figsetplot{604918900665305600.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.207}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604919136887960704}
\figsetplot{604919136887960704.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.208}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604919278622426624}
\figsetplot{604919278622426624.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.209}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604919617924301184}
\figsetplot{604919617924301184.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.210}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604920171975748224}
\figsetplot{604920171975748224.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.211}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604920339478833536}
\figsetplot{604920339478833536.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.212}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604920412493792384}
\figsetplot{604920412493792384.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.213}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604920549932807296}
\figsetplot{604920549932807296.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.214}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604920549932809472}
\figsetplot{604920549932809472.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.215}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604920584291606144}
\figsetplot{604920584291606144.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.216}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604920653011055104}
\figsetplot{604920653011055104.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.217}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604920751795652864}
\figsetplot{604920751795652864.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.218}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604920893530008064}
\figsetplot{604920893530008064.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.219}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604921164112524800}
\figsetplot{604921164112524800.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.220}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604921713868728448}
\figsetplot{604921713868728448.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.221}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604922027401371904}
\figsetplot{604922027401371904.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.222}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604922057465857792}
\figsetplot{604922057465857792.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.223}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604922229264424448}
\figsetplot{604922229264424448.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.224}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604922297983905920}
\figsetplot{604922297983905920.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.225}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604922370997734016}
\figsetplot{604922370997734016.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.226}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604922847739721856}
\figsetplot{604922847739721856.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.227}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604922847739724800}
\figsetplot{604922847739724800.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.228}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604922886394970240}
\figsetplot{604922886394970240.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.229}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604922920754526080}
\figsetplot{604922920754526080.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.230}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604922955113458432}
\figsetplot{604922955113458432.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.231}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604923092553224320}
\figsetplot{604923092553224320.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.232}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604923126912957952}
\figsetplot{604923126912957952.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.233}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604923191337116672}
\figsetplot{604923191337116672.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.234}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604923848467470976}
\figsetplot{604923848467470976.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.235}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604924088985646464}
\figsetplot{604924088985646464.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.236}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604924088985647360}
\figsetplot{604924088985647360.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.237}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604924157705123072}
\figsetplot{604924157705123072.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.238}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604924226424592768}
\figsetplot{604924226424592768.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.239}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604924531366934784}
\figsetplot{604924531366934784.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.240}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604924604381692160}
\figsetplot{604924604381692160.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.241}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604924707462709120}
\figsetplot{604924707462709120.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.242}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604924737525369344}
\figsetplot{604924737525369344.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.243}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604924840604588416}
\figsetplot{604924840604588416.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.244}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604925046762260096}
\figsetplot{604925046762260096.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.245}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604925390359645056}
\figsetplot{604925390359645056.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.246}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604926184929812224}
\figsetplot{604926184929812224.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.247}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604926592950492160}
\figsetplot{604926592950492160.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.248}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604927039627095040}
\figsetplot{604927039627095040.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.249}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604927421880381184}
\figsetplot{604927421880381184.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.250}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604928036059785088}
\figsetplot{604928036059785088.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.251}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604928139138729344}
\figsetplot{604928139138729344.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.252}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604929620903657856}
\figsetplot{604929620903657856.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.253}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604929655263400832}
\figsetplot{604929655263400832.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.254}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604929689624751488}
\figsetplot{604929689624751488.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.255}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604930681760052096}
\figsetplot{604930681760052096.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.256}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604930681760054656}
\figsetplot{604930681760054656.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.257}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604932124868388224}
\figsetplot{604932124868388224.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.258}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604933121300811520}
\figsetplot{604933121300811520.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.259}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604938550139479680}
\figsetplot{604938550139479680.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.260}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604938859377130880}
\figsetplot{604938859377130880.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.261}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604938859377134080}
\figsetplot{604938859377134080.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.262}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604939271694093440}
\figsetplot{604939271694093440.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.263}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604942540165288960}
\figsetplot{604942540165288960.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.264}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604942570229541120}
\figsetplot{604942570229541120.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.265}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604944361231413760}
\figsetplot{604944361231413760.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.266}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604945288944333440}
\figsetplot{604945288944333440.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.267}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604945559526273536}
\figsetplot{604945559526273536.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.268}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604945976139106560}
\figsetplot{604945976139106560.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.269}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604946865196192000}
\figsetplot{604946865196192000.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.270}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604946865196193280}
\figsetplot{604946865196193280.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.271}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604946938211616000}
\figsetplot{604946938211616000.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.272}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604947006931096320}
\figsetplot{604947006931096320.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.273}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604947140074786816}
\figsetplot{604947140074786816.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.274}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604947449312435072}
\figsetplot{604947449312435072.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.275}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604947827269657472}
\figsetplot{604947827269657472.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.276}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604948342665639040}
\figsetplot{604948342665639040.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.277}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604948583183812864}
\figsetplot{604948583183812864.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.278}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604949102875105536}
\figsetplot{604949102875105536.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.279}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604949923212906880}
\figsetplot{604949923212906880.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.280}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604949927508816768}
\figsetplot{604949927508816768.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.281}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604950236746474880}
\figsetplot{604950236746474880.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.282}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604950545984126080}
\figsetplot{604950545984126080.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.283}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604951297602424320}
\figsetplot{604951297602424320.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.284}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604951297602581888}
\figsetplot{604951297602581888.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.285}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604951542415727744}
\figsetplot{604951542415727744.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.286}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604960334214210688}
\figsetplot{604960334214210688.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.287}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604960609092130688}
\figsetplot{604960609092130688.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.288}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604960609092133248}
\figsetplot{604960609092133248.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.289}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604961742964300672}
\figsetplot{604961742964300672.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.290}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604961777323248384}
\figsetplot{604961777323248384.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.291}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604962292719320832}
\figsetplot{604962292719320832.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.292}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604962533237909120}
\figsetplot{604962533237909120.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.293}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604962709331635072}
\figsetplot{604962709331635072.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.294}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604963259087437184}
\figsetplot{604963259087437184.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.295}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604963911922477696}
\figsetplot{604963911922477696.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.296}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604964010707107840}
\figsetplot{604964010707107840.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.297}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604964079425764736}
\figsetplot{604964079425764736.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.298}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604964148145244800}
\figsetplot{604964148145244800.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.299}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604964251224459520}
\figsetplot{604964251224459520.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.300}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604964285584199680}
\figsetplot{604964285584199680.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.301}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604964354309369728}
\figsetplot{604964354309369728.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.302}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604964461678281600}
\figsetplot{604964461678281600.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.303}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604965522534367616}
\figsetplot{604965522534367616.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.304}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604965934851301632}
\figsetplot{604965934851301632.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.305}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604966003570704256}
\figsetplot{604966003570704256.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.306}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604966450248346880}
\figsetplot{604966450248346880.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.307}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604966518966784256}
\figsetplot{604966518966784256.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.308}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604966763780773248}
\figsetplot{604966763780773248.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.309}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604966828204831616}
\figsetplot{604966828204831616.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.310}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604967206161971200}
\figsetplot{604967206161971200.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.311}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604967588414483712}
\figsetplot{604967588414483712.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.312}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604967858996581120}
\figsetplot{604967858996581120.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.313}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604967966371608576}
\figsetplot{604967966371608576.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.314}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604968133874491392}
\figsetplot{604968133874491392.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.315}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604968172529056384}
\figsetplot{604968172529056384.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.316}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604968206888780032}
\figsetplot{604968206888780032.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.317}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604968236953708416}
\figsetplot{604968236953708416.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.318}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604968408756601088}
\figsetplot{604968408756601088.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.319}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604968791005321216}
\figsetplot{604968791005321216.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.320}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604968958508607360}
\figsetplot{604968958508607360.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.321}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604969267746267520}
\figsetplot{604969267746267520.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.322}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604969615638992896}
\figsetplot{604969615638992896.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.323}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604969856157171584}
\figsetplot{604969856157171584.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.324}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604969954941056384}
\figsetplot{604969954941056384.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.325}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604970058020251520}
\figsetplot{604970058020251520.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.326}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604970062315630336}
\figsetplot{604970062315630336.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.327}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604970131035099008}
\figsetplot{604970131035099008.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.328}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604970302833797376}
\figsetplot{604970302833797376.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.329}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604970435977387520}
\figsetplot{604970435977387520.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.330}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604970715150627456}
\figsetplot{604970715150627456.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.331}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604970783870102912}
\figsetplot{604970783870102912.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.332}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604970921309072640}
\figsetplot{604970921309072640.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.333}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604971402345380480}
\figsetplot{604971402345380480.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.334}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604971677223267072}
\figsetplot{604971677223267072.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.335}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604971745942742656}
\figsetplot{604971745942742656.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.336}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604971849020954624}
\figsetplot{604971849020954624.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.337}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604971917741440640}
\figsetplot{604971917741440640.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.338}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604972089540122368}
\figsetplot{604972089540122368.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.339}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604972394482497280}
\figsetplot{604972394482497280.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.340}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604972394482498304}
\figsetplot{604972394482498304.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.341}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604973562713585792}
\figsetplot{604973562713585792.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.342}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604974078109680000}
\figsetplot{604974078109680000.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.343}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604974078113845120}
\figsetplot{604974078113845120.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.344}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604974284268110720}
\figsetplot{604974284268110720.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.345}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604974529083276800}
\figsetplot{604974529083276800.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.346}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604974597801096064}
\figsetplot{604974597801096064.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.347}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604974769599793152}
\figsetplot{604974769599793152.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.348}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604975383780541952}
\figsetplot{604975383780541952.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.349}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604976139698283008}
\figsetplot{604976139698283008.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.350}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604976418867174528}
\figsetplot{604976418867174528.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.351}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604977071702226688}
\figsetplot{604977071702226688.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.352}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604977312220363776}
\figsetplot{604977312220363776.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.353}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604982358806179456}
\figsetplot{604982358806179456.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.354}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604982736763369856}
\figsetplot{604982736763369856.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.355}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604982805482785152}
\figsetplot{604982805482785152.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.356}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604984935786576896}
\figsetplot{604984935786576896.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.357}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604987547126699264}
\figsetplot{604987547126699264.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.358}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604987826300371712}
\figsetplot{604987826300371712.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.359}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604988612278594048}
\figsetplot{604988612278594048.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.360}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604988685293803520}
\figsetplot{604988685293803520.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.361}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604990197122292224}
\figsetplot{604990197122292224.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.362}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604993869318584960}
\figsetplot{604993869318584960.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.363}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604995278068254208}
\figsetplot{604995278068254208.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.364}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604996106997220480}
\figsetplot{604996106997220480.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.365}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604996137063022336}
\figsetplot{604996137063022336.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.366}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604996141358671744}
\figsetplot{604996141358671744.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.367}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604996583742879616}
\figsetplot{604996583742879616.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.368}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604996588033758208}
\figsetplot{604996588033758208.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.369}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604996618098066432}
\figsetplot{604996618098066432.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.370}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604996622395017472}
\figsetplot{604996622395017472.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.371}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604996725474241280}
\figsetplot{604996725474241280.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.372}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604996927335710080}
\figsetplot{604996927335710080.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.373}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604997240868589824}
\figsetplot{604997240868589824.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.374}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604999882273217152}
\figsetplot{604999882273217152.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.375}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604999886568459136}
\figsetplot{604999886568459136.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.376}
\figsetgrptitle{Light curve and periodogram of Gaia ID 604999886568459392}
\figsetplot{604999886568459392.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.377}
\figsetgrptitle{Light curve and periodogram of Gaia ID 605000058367154176}
\figsetplot{605000058367154176.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.378}
\figsetgrptitle{Light curve and periodogram of Gaia ID 605002802850299264}
\figsetplot{605002802850299264.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.379}
\figsetgrptitle{Light curve and periodogram of Gaia ID 605004834370703744}
\figsetplot{605004834370703744.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.380}
\figsetgrptitle{Light curve and periodogram of Gaia ID 605012870254630912}
\figsetplot{605012870254630912.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.381}
\figsetgrptitle{Light curve and periodogram of Gaia ID 605014141564219776}
\figsetplot{605014141564219776.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.382}
\figsetgrptitle{Light curve and periodogram of Gaia ID 605014214579367424}
\figsetplot{605014214579367424.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetgrpstart
\figsetgrpnum{16.383}
\figsetgrptitle{Light curve and periodogram of Gaia ID 607994986306236928}
\figsetplot{607994986306236928.pdf}
\figsetgrpnote{Light curves and periodograms for all sources in the rotation catalog. In the top left is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines.}
\figsetgrpend

\figsetend

\begin{figure}
    \gridline{\fig{lc_example1.pdf}{1.0\textwidth}{}}
    \gridline{\fig{lc_example2.pdf}{1.0\textwidth}{}}
    %\includegraphics{}
    \caption{Example light curves and periodograms for select cluster members. In the top left of each target's set is the light curve of the target. Bottom left is the phase-folded version, folded on the period of max power in the periodogram. On the right, the periodogram and a subset centered on the period of max power. Window peaks are denoted with vertical dotted lines. The complete figure set (594 images) is available in the online journal.}
    \label{fig:example_lcs}
\end{figure}



